Braided Quantum Field Theory

We develop a general framework for quantum field theory on noncommutative spaces, i.e., spaces with quantum group symmetry. We use the path integral approach to obtain expressions for $n$-point functions. Perturbation theory leads us to generalised Feynman diagrams which are braided, i.e., they have non-trivial over- and under-crossings. We demonstrate the power of our approach by applying it to $\phi^4$-theory on the quantum 2-sphere. We find that the basic divergent diagram of the theory is regularised.

==> fig_free6r.tex <==
$\begin{array}{cccccc}
&
\sxy{
(10,10)**\crv{(0,10)},
(20,10);(30,0)**\crv{(30,10)},
\vunder~{(10,10)}{(20,10)}{(10,0)}{(20,0)},
(40,0);(50,0)**\crv{(40,10)&(50,10)}}
& + &
\sxy{
(10,10)**\crv{(0,10)},
\vunder~{(10,10)}{(20,10)}{(10,0)}{(20,0)},
(20,10);(30,10)**\dir{-},
\vunder~{(30,10)}{(40,10)}{(30,0)}{(40,0)},
(40,10);(50,0)**\crv{(50,10)}}
& + &
\sxy{
(10,8)**\crv{(0,6)},
\vunder~{(10,8)}{(20,10)}{(10,0)}{(20,0)},
(20,10);(50,0)**\crv{(50,16)},
(30,0);(40,0)**\crv{(30,10)&(40,10)}}
\\ + &
\sxy{
(30,0)**\crv{(0,15)&(30,15)},
(10,0);(20,0)**\crv{(10,10)&(20,10)},
(40,0);(50,0)**\crv{(40,10)&(50,10)}}
& + &
\sxy{
(10,8)**\crv{(0,4)},
\vunder~{(10,8)}{(15,10)}{(10,0)}{(20,10)},
(15,10);(35,10)**\crv{(25,14)},
\vunder~{(20,10)}{(30,10)}{(20,0)}{(30,0)},
\vunder~{(35,10)}{(40,8)}{(30,10)}{(40,0)},
(40,8);(50,0)**\crv{(50,4)}}
& + &
\sxy{
(10,10)**\crv{(0,8)},
\vunder~{(10,10)}{(15,11)}{(10,0)}{(20,10)},
\vunder~{(20,10)}{(30,8)}{(20,0)}{(30,0)},
(15,11);(50,0)**\crv{(50,18)},
(30,8);(40,0)**\crv{(40,6)}}
\\ + &
\sxy{
(30,10)**\crv{(0,16)},
(10,0);(20,0)**\crv{(10,10)&(20,10)},
\vunder~{(30,10)}{(40,8)}{(30,0)}{(40,0)},
(50,0);(40,8)**\crv{(50,6)}}
& + &
\sxy{
(35,11)**\crv{(0,18)},
(10,0);(20,8)**\crv{(10,6)},
\vunder~{(20,8)}{(30,10)}{(20,0)}{(30,0)},
\vunder~{(35,11)}{(40,10)}{(30,10)}{(40,0)},
(40,10);(50,0)**\crv{(50,8)}}
& + &
\sxy{
(10,12)**\crv{(0,12)},
\vunder~{(10,12)}{(40,12)}{(10,0)}{(40,0)},
(50,0);(40,12)**\crv{(50,12)},
(20,0);(30,0)**\crv{(20,10)&(30,10)}}
\\ + &
\sxy{
(50,0)**\crv{(0,15)&(50,15)},
(10,0);(20,0)**\crv{(10,10)&(20,10)},
(30,0);(40,0)**\crv{(30,10)&(40,10)}}
& + &
\sxy{
(50,0)**\crv{(0,20)&(50,20)},
(10,0);(20,10)**\crv{(10,10)},
\vunder~{(20,10)}{(30,10)}{(20,0)}{(30,0)},
(30,10);(40,0)**\crv{(40,10)}}
& + &
\sxy{
(50,0)**\crv{(0,20)&(50,20)},
(10,0);(40,0)**\crv{(10,15)&(40,15)},
(20,0);(30,0)**\crv{(20,10)&(30,10)}}
\end{array}$

